TDM: Temporally-Consistent Diffusion Model for All-in-One Real-World Video Restoration

In this paper, we propose the first diffusion-based all-in-one video restoration method that utilizes the power of a pre-trained Stable Diffusion and a fine-tuned ControlNet. Our method can restore various types of video degradation with a single unified model, overcoming the limitation of standard methods that require specific models for each restoration task. Our contributions include an efficient training strategy with Task Prompt Guidance (TPG) for diverse restoration tasks, an inference strategy that combines Denoising Diffusion Implicit Models~(DDIM) inversion with a novel Sliding Window Cross-Frame Attention (SW-CFA) mechanism for enhanced content preservation and temporal consistency, and a scalable pipeline that makes our method all-in-one to adapt to different video restoration tasks. Through extensive experiments on five video restoration tasks, we demonstrate the superiority of our method in generalization capability to real-world videos and temporal consistency preservation over existing state-of-the-art methods. Our method advances the video restoration task by providing a unified solution that enhances video quality across multiple applications.

==> Sections/related_works.tex <==
\section{Related Works} \label{sec:related_work}
\textbf{Task-Specific Image and Video Restoration.}
Task-specific image restoration aims to recover a clean image from the degraded observation which is corrupted by only a specific degradation type, such as image denoising~\cite{DnCNN,niknejad2017class,FFDNet,MIRNet,NBNet}, deraining~\cite{Removing_Rain2017,jiang2020multi,li2018recurrent,li2022dual,li2022single,wu2021contrastive}, dehazing~\cite{MixDehazeNet,C2PNet,gUNet-D,FFANet,DEA-Net}, super-resolution~\cite{HAT-L,SwinFIR,DAT+,RGT+,DBPN-RESMR643}, etc.  Despite the significant advancements in single-image-based image restoration techniques, challenges persist in processing video data due to the inherent nature of frame-by-frame processing, which frequently results in temporal inconsistency within the processed video results. To address these issues, numerous video restoration models~\cite{Basicvsr,Restore_from_restored,temporal_dynamics_videos,efficient_multi_stage_video,Cascaded_Deep_Video,Patch_Craft,Sharpness_Feature_From_Exemplars} have been developed and proposed.~Huang et al.~\cite{huang2015bidirectional} propose a bidirectional recurrent convolutional neural network for super-resolution. Cao et al.~\cite{cao2022learning} further extract multi-scale optical flows to take advantage of the flow guidance by progressively introducing and refining more flow information from low resolution to high resolution. MAP-Net~\cite{MAP_Net} introduces a novel framework to effectively explore the physical haze priors and aggregate temporal information. Although the existing image and video restoration methods achieve impressive results on specific tasks, their ability to generalize across different types of degradation remains limited. Some studies~\cite{vrt,rvrt,Restormer} demonstrate adaptability to various degradations; however, they require training separate models for different tasks, contrary to the practical need for a single unified model.

\noindent\textbf{Multi-Task Image Restoration.} Recently, multi-task image restoration has gained increased interest due to its ability to address a broad spectrum of restoration tasks using a single network. Extensive research has been conducted on restoring images degraded by various weather conditions such as snow, fog, and rain, as detailed in studies~\cite{weather_general,AIOWeather}. These methods typically enhance the images through the training of specialized encoders tailored to each specific weather degradation condition. AirNet~\cite{airnet} introduces an all-in-one image restoration network which consists of a contrastive-based degraded encoder for task-specific feature representation learning and a degradation-guided restoration network for multiple-type image restoration. Potlapalli et.al~\cite{promptir} use prompts to encode degradation-specific information, which is then used to guide the restoration network dynamically. This prompt learning approach enables the network to generalize across different types and levels of degradation. While these methods move towards a general restoration model for practical use, they remain designed for single images and may fail to maintain temporal consistency in video applications, lacking the ability to fully leverage multi-frame information.  How to develop an all-in-one restoration model for video is still a problem that has yet to be explored.


\noindent\textbf{Diffusion-Base Image Restoration.}
With rapid advancements in generative AI, especially diffusion models, numerous studies have investigated using diffusion models for image restoration tasks. Instructpix2pix~\cite{instructpix2pix} was among the first to adapt the SD model~\cite{LatentDiffusion}  for image editing tasks, by providing an input image along with a text prompt directing the model's actions. Additionally, several diffusion models specifically designed for low-level tasks have been developed~\cite{weatherdiffusion,diffplugin,upscale_diff_vid_sr}. Legenstein et al. proposed a novel patch-based image restoration algorithm using Denoising Diffusion Probabilistic Models (DDPM) for tasks such as image desnowing, combined draining and dehazing, and raindrop removal. Diff-Plugin~\cite{diffplugin} further proposes a framework to enable a single pre-trained diffusion model to generate high-fidelity results across a variety of low-level tasks using a plugin selector that can automatically select different task plugins based on the text instructions. Moreover, due to the tendency of large pre-trained diffusion models to introduce artifacts into the original image content, several approaches have been developed to maintain content consistency, especially when processing sequential images such as videos. Text2Video-zero~\cite{Text2Video-zero} leverages the motion dynamics between the latent codes of the current and initial frames to maintain global scene time consistency and employs a cross-frame attention mechanism to preserve the appearance and identity of the foreground object.  However, its temporal consistency depends entirely on the initial frame, limiting its effectiveness for longer videos and significant motion.  ControlVideo~\cite{controlvideo} enhances performance by utilizing structural consistency from input motion sequences and integrating complete cross-frame interaction within self-attention modules. However, this approach substantially increases computational complexity and memory usage.
